Dissections of trapezoids into trapezoids homothetic to trapezoids of a given set

Here I present several theorems about trapezoids tilings. The first one is related to trapezoids with rational base relation, the other ones are related to those with base relation from quadratic number field.

==> pic1.tex <==

\definecolor{xdxdff}{rgb}{0.49019607843137253,0.49019607843137253,1.}
\definecolor{qqqqff}{rgb}{0.,0.,1.}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.23cm,y=0.23cm]
\clip(-27.58308727564073,-7.20699131930134) rectangle (77.70795142124715,37.22915236767604);
\draw (20.,8.)-- (21.,6.);
\draw (20.,8.)-- (24.,8.);
\draw (24.,8.)-- (23.,6.);
\draw (24.,8.)-- (26.,8.);
\draw (26.,8.)-- (27.,6.);
\draw (21.,6.)-- (22.,4.);
\draw (21.,6.)-- (25.,6.);
\draw (25.,6.)-- (24.,4.);
\draw (25.,6.)-- (27.,6.);
\draw (27.,6.)-- (28.,4.);
\draw (22.,4.)-- (23.,2.);
\draw (22.,4.)-- (26.,4.);
\draw (26.,4.)-- (25.,2.);
\draw (26.,4.)-- (28.,4.);
\draw (28.,4.)-- (29.,2.);
\draw (23.,2.)-- (24.,0.);
\draw (23.,2.)-- (27.,2.);
\draw (27.,2.)-- (26.,0.);
\draw (27.,2.)-- (29.,2.);
\draw (29.,2.)-- (30.,0.);
\draw (24.,0.)-- (25.,-2.);
\draw (24.,0.)-- (28.,0.);
\draw (28.,0.)-- (27.,-2.);
\draw (28.,0.)-- (30.,0.);
\draw (30.,0.)-- (31.,-2.);
\draw (25.,-2.)-- (26.,-4.);
\draw (25.,-2.)-- (29.,-2.);
\draw (29.,-2.)-- (28.,-4.);
\draw (29.,-2.)-- (31.,-2.);
\draw (31.,-2.)-- (32.,-4.);
\draw (14.,20.)-- (15.,18.);
\draw (14.,20.)-- (18.,20.);
\draw (18.,20.)-- (17.,18.);
\draw (18.,20.)-- (20.,20.);
\draw (20.,20.)-- (21.,18.);
\draw (15.,18.)-- (16.,16.);
\draw (15.,18.)-- (19.,18.);
\draw (19.,18.)-- (18.,16.);
\draw (19.,18.)-- (21.,18.);
\draw (21.,18.)-- (22.,16.);
\draw (16.,16.)-- (17.,14.);
\draw (16.,16.)-- (20.,16.);
\draw (20.,16.)-- (19.,14.);
\draw (20.,16.)-- (22.,16.);
\draw (22.,16.)-- (23.,14.);
\draw (17.,14.)-- (18.,12.);
\draw (17.,14.)-- (21.,14.);
\draw (21.,14.)-- (20.,12.);
\draw (21.,14.)-- (23.,14.);
\draw (23.,14.)-- (24.,12.);
\draw (18.,12.)-- (19.,10.);
\draw (18.,12.)-- (22.,12.);
\draw (22.,12.)-- (21.,10.);
\draw (22.,12.)-- (24.,12.);
\draw (24.,12.)-- (25.,10.);
\draw (19.,10.)-- (20.,8.);
\draw (19.,10.)-- (23.,10.);
\draw (23.,10.)-- (22.,8.);
\draw (23.,10.)-- (25.,10.);
\draw (25.,10.)-- (26.,8.);
\draw (-4.,32.)-- (8.,32.);
\draw (-4.,32.)-- (-10.,20.);
\draw (-10.,20.)-- (14.,20.);
\draw (8.,32.)-- (9.,30.);
\draw (8.,32.)-- (12.,32.);
\draw (12.,32.)-- (11.,30.);
\draw (12.,32.)-- (14.,32.);
\draw (14.,32.)-- (15.,30.);
\draw (9.,30.)-- (10.,28.);
\draw (9.,30.)-- (13.,30.);
\draw (13.,30.)-- (12.,28.);
\draw (13.,30.)-- (15.,30.);
\draw (15.,30.)-- (16.,28.);
\draw (10.,28.)-- (11.,26.);
\draw (10.,28.)-- (14.,28.);
\draw (14.,28.)-- (13.,26.);
\draw (14.,28.)-- (16.,28.);
\draw (16.,28.)-- (17.,26.);
\draw (11.,26.)-- (12.,24.);
\draw (11.,26.)-- (15.,26.);
\draw (15.,26.)-- (14.,24.);
\draw (15.,26.)-- (17.,26.);
\draw (17.,26.)-- (18.,24.);
\draw (12.,24.)-- (13.,22.);
\draw (12.,24.)-- (16.,24.);
\draw (16.,24.)-- (15.,22.);
\draw (16.,24.)-- (18.,24.);
\draw (18.,24.)-- (19.,22.);
\draw (13.,22.)-- (14.,20.);
\draw (13.,22.)-- (17.,22.);
\draw (17.,22.)-- (16.,20.);
\draw (17.,22.)-- (19.,22.);
\draw (19.,22.)-- (20.,20.);
\draw (26.,-4.)-- (28.,-4.);
\draw (28.,-4.)-- (32.,-4.);
\draw (-10.,20.)-- (-22.,-4.);
\draw (-22.,-4.)-- (26.,-4.);
\draw [dotted] (-10.,20.)-- (-10.07858677650699,-4.);
\draw [dotted] (-4.,32.)-- (-4.025725561222746,20.);
\draw (-4.,32.)-- (14.,32.);
\draw (-22.,-4.)-- (32.,-4.);
\draw [dotted] (14.,32.)-- (22.,32.);
\draw [dotted] (15.,30.)-- (22.,30.);
\draw (22.,30.)-- (22.,32.);
\begin{scriptsize}
\draw[color=black] (3.131693005320853,31.072579826091996) node {$\frac13$};
\draw[color=black] (3.5478110782330265,18.92193209705643) node {$\frac23$};
\draw[color=black] (9.705041932322423,33.23441886771915) node {$\frac19$};
\draw[color=black] (12.701092057290076,33.23441886771915) node {$\frac1{18}$};
\draw[color=black] (5.0471527657276365,-2.4181826318929279) node {$\frac43$};
\draw[color=black] (-7.2752086925158466,9.10088726382367) node {$\frac23(\frac{\sqrt 3}2)$};
\draw[color=black] (-2.0665624011667653,26.74429355529997) node {$\frac13(\frac{\sqrt 3}2)$};
\draw[color=black] (4.129059755299289,33.23441886771915) node {$\frac12$};
\draw[color=black] (7.210966744870942,-5.212916131849826) node {$\frac32$};
\draw[color=black] (24.76456629671078,31.43771043024609) node {$\frac1{18}(\frac{\sqrt3}2)$};
\end{scriptsize}
\end{tikzpicture}

==> pic2.tex <==
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.35cm,y=0.35cm]
\clip(-4.327613052815176,-0.8090588245869035) rectangle (48.99046392025017,21.26746589010648);
\draw (6.,1.)-- (9.,7.);
\draw (9.,7.)-- (15.,7.);
\draw (15.,7.)-- (18.,1.);
\draw (18.,1.)-- (6.,1.);
\draw (15.,7.)-- (29.,7.);
\draw (29.,7.)-- (26.,1.);
\draw (18.,1.)-- (26.,1.);
\draw (29.,7.)-- (37.,7.);
\draw (37.,7.)-- (40.,1.);
\draw (40.,1.)-- (26.,1.);
\draw (37.,7.)-- (30.,21.);
\draw (9.,7.)-- (16.,21.);
\draw (16.,21.)-- (30.,21.);
\draw [dotted] (2.,7.)-- (9.,7.);
\draw [dotted] (2.,1.)-- (6.,1.);
\draw [dotted] (2.,21.)-- (16.,21.);
\draw (2.,21.)-- (2.,7.);
\draw (2.,7.)-- (2.,1.);
\draw (9.,7.)-- (37.,7.);
\draw (6.,1.)-- (40.,1.);
\begin{scriptsize}
\draw[color=black] (12.061079942280307,6.1559086011819115) node {$1-\frac{\sqrt2}{2}$};
\draw[color=black] (11.806377892189854,1.5855330507899668) node {$2-\sqrt2$};
\draw[color=black] (22.073127986863227,6.1559086011819115) node {$\frac{\sqrt2}{2}$};
\draw[color=black] (21.282101449295386,1.6792636506693681) node {$\sqrt2-1$};
\draw[color=black] (32.31252705649137,6.1559086011819115) node {$\sqrt2-1$};
\draw[color=black] (33.10355359405921,2.0855330507899668) node {$\frac{\sqrt2}{2}$};
\draw[color=black] (23.052046361938603,19.974656683634126) node {$\frac{\sqrt2}2$};
\draw[color=black] (0.066057429154677,14.390390301845203) node {$\frac{\sqrt 2}{2}\left(\frac{\sqrt3}{2}\right)$};
\draw[color=black] (-1.643623773074275,4.37072082598594) node {$\left(1-\frac{\sqrt 2}{2}\right)\left(\frac{\sqrt3}{2}\right)$};
\draw[color=black] (22.161019824370765,7.6559086011819115) node {$\sqrt 2$};
\draw[color=black] (21.34755963072252,0.0) node {$1+\frac{\sqrt2}{2}$};
\end{scriptsize}
\end{tikzpicture}
